Probing the $\tau$ anomalous magnetic and electric dipole moments in photon-induced $\gamma\gamma\to\tau^+\tau^-$ production at the FCC-hh

The sensitivity of the FCC-hh to the anomalous magnetic moment $a_\tau$ and the electric dipole moment $d_\tau$ of the $\tau$ lepton is studied in photon-induced $\gamma\gamma\to\tau^+\tau^-$ production with both $\tau$ leptons decaying hadronically. Central exclusive (elastic) signal events, in which both protons remain intact, are generated with MadGraph5_aMC@NLO using a FeynRules UFO model of the anomalous $\gamma\tau\tau$ vertex merged with the TauDecay model, so that the $\tau$ decays and their spin correlations are included in the matrix element. Single- and double-dissociative production is estimated with SuperChic and added to the elastic signal with its own coupling dependence and with normalisation and shape uncertainties of 25%. Pythia 8 decays the unstable hadrons in the signal, decays the $\tau$ leptons and simulates the parton shower and hadronisation in the backgrounds, and hadronises the dissociated protons. Signal and backgrounds are passed through the Delphes simulation of the FCC-hh detector. Hadronic $\tau$ decays are reconstructed from particle-flow tracks and photons with an algorithm based on the hadrons-plus-strips approach, with an efficiency of 73.4% within the acceptance. Requiring no additional tracks from the $\tau$ vertices retains part of the dissociative contribution and reduces the Drell-Yan and $\gamma\gamma\to WW$ backgrounds to 0.9% of the SM yield. The couplings are constrained from the shape of the total transverse mass distribution. For a centre-of-mass energy of 84 TeV and 30 ab$^{-1}$, the expected 95% CL limits are $-3.38\times10^{-4} < a_\tau < 3.36\times10^{-4}$ and $|d_\tau| < 1.88\times10^{-18}\,e\,$cm, about an order of magnitude beyond the current bounds. Results are also given for FCC-hh scenarios between 72 and 120 TeV and for an optimistic detector parametrisation.

==> q/numbers.tex <==
% OTOMATİK: scripts/paper/make_numbers.py — elle düzenlemeyin
% d_τ: 10^{-18} e cm; a_τ: 10^{-4}; yüzdeler: %
\makeatletter
\@namedef{res@CNP-max}{2.5}
\@namedef{res@CNP-min}{1.7}
\@namedef{res@CSM-max}{2.2}
\@namedef{res@CSM-min}{1.8}
\@namedef{res@K-eff-absmax}{1.2}
\@namedef{res@K-eff-max}{+0.1}
\@namedef{res@K-eff-min}{-1.2}
\@namedef{res@K-low-dev}{5}
\@namedef{res@K-max}{1.10}
\@namedef{res@K-min}{0.91}
\@namedef{res@atau-102-0.3}{9.4}
\@namedef{res@atau-102-1}{7.0}
\@namedef{res@atau-102-10}{4.0}
\@namedef{res@atau-102-3}{5.3}
\@namedef{res@atau-102-30}{3.1}
\@namedef{res@atau-102-9.2}{4.1}
\@namedef{res@atau-120-0.3}{8.6}
\@namedef{res@atau-120-1}{6.3}
\@namedef{res@atau-120-10}{3.5}
\@namedef{res@atau-120-3}{4.8}
\@namedef{res@atau-120-3.7}{4.5}
\@namedef{res@atau-120-30}{2.7}
\@namedef{res@atau-72-0.3}{11.0}
\@namedef{res@atau-72-1}{8.2}
\@namedef{res@atau-72-10}{4.8}
\@namedef{res@atau-72-20}{4.1}
\@namedef{res@atau-72-3}{6.3}
\@namedef{res@atau-72-30}{3.7}
\@namedef{res@atau-72-9.5}{4.9}
\@namedef{res@atau-84-0.3}{10.2}
\@namedef{res@atau-84-1}{7.6}
\@namedef{res@atau-84-10}{4.4}
\@namedef{res@atau-84-3}{5.8}
\@namedef{res@atau-84-30}{3.4}
\@namedef{res@atau-84-9.2}{4.5}
\@namedef{res@atauEL-102-0.3}{11.5}
\@namedef{res@atauEL-102-1}{8.3}
\@namedef{res@atauEL-102-10}{4.5}
\@namedef{res@atauEL-102-3}{6.2}
\@namedef{res@atauEL-102-30}{3.5}
\@namedef{res@atauEL-102-9.2}{4.6}
\@namedef{res@atauEL-120-0.3}{10.7}
\@namedef{res@atauEL-120-1}{7.6}
\@namedef{res@atauEL-120-10}{4.1}
\@namedef{res@atauEL-120-3}{5.6}
\@namedef{res@atauEL-120-3.7}{5.3}
\@namedef{res@atauEL-120-30}{3.1}
\@namedef{res@atauEL-72-0.3}{13.2}
\@namedef{res@atauEL-72-1}{9.5}
\@namedef{res@atauEL-72-10}{5.3}
\@namedef{res@atauEL-72-20}{4.5}
\@namedef{res@atauEL-72-3}{7.1}
\@namedef{res@atauEL-72-30}{4.1}
\@namedef{res@atauEL-72-9.5}{5.3}
\@namedef{res@atauEL-84-0.3}{12.2}
\@namedef{res@atauEL-84-1}{8.7}
\@namedef{res@atauEL-84-10}{4.9}
\@namedef{res@atauEL-84-3}{6.5}
\@namedef{res@atauEL-84-30}{3.7}
\@namedef{res@atauEL-84-9.2}{5.0}
\@namedef{res@atauclip1-102}{14.7}
\@namedef{res@atauclip1-120}{14.4}
\@namedef{res@atauclip1-72}{15.7}
\@namedef{res@atauclip1-84}{14.5}
\@namedef{res@atauclip2-102}{9.4}
\@namedef{res@atauclip2-120}{9.0}
\@namedef{res@atauclip2-72}{9.7}
\@namedef{res@atauclip2-84}{9.7}
\@namedef{res@atauclip3-102}{7.3}
\@namedef{res@atauclip3-120}{7.2}
\@namedef{res@atauclip3-72}{7.9}
\@namedef{res@atauclip3-84}{7.5}
\@namedef{res@atauclip5-102}{5.4}
\@namedef{res@atauclip5-120}{5.0}
\@namedef{res@atauclip5-72}{5.9}
\@namedef{res@atauclip5-84}{5.5}
\@namedef{res@atauclip8-102}{4.5}
\@namedef{res@atauclip8-120}{4.1}
\@namedef{res@atauclip8-72}{5.1}
\@namedef{res@atauclip8-84}{4.7}
\@namedef{res@atauhi-102-0.3}{9.34}
\@namedef{res@atauhi-102-1}{6.94}
\@namedef{res@atauhi-102-10}{3.97}
\@namedef{res@atauhi-102-3}{5.33}
\@namedef{res@atauhi-102-30}{3.04}
\@namedef{res@atauhi-102-9.2}{4.06}
\@namedef{res@atauhi-120-0.3}{8.63}
\@namedef{res@atauhi-120-1}{6.33}
\@namedef{res@atauhi-120-10}{3.51}
\@namedef{res@atauhi-120-3}{4.78}
\@namedef{res@atauhi-120-3.7}{4.52}
\@namedef{res@atauhi-120-30}{2.67}
\@namedef{res@atauhi-72-0.3}{10.96}
\@namedef{res@atauhi-72-1}{8.20}
\@namedef{res@atauhi-72-10}{4.80}
\@namedef{res@atauhi-72-20}{4.08}
\@namedef{res@atauhi-72-3}{6.35}
\@namedef{res@atauhi-72-30}{3.71}
\@namedef{res@atauhi-72-9.5}{4.86}
\@namedef{res@atauhi-84-0.3}{10.16}
\@namedef{res@atauhi-84-1}{7.59}
\@namedef{res@atauhi-84-10}{4.36}
\@namedef{res@atauhi-84-3}{5.84}
\@namedef{res@atauhi-84-30}{3.36}
\@namedef{res@atauhi-84-9.2}{4.45}
\@namedef{res@ataulo-102-0.3}{-9.44}
\@namedef{res@ataulo-102-1}{-7.01}
\@namedef{res@ataulo-102-10}{-3.98}
\@namedef{res@ataulo-102-3}{-5.35}
\@namedef{res@ataulo-102-30}{-3.05}
\@namedef{res@ataulo-102-9.2}{-4.06}
\@namedef{res@ataulo-120-0.3}{-8.55}
\@namedef{res@ataulo-120-1}{-6.28}
\@namedef{res@ataulo-120-10}{-3.54}
\@namedef{res@ataulo-120-3}{-4.77}
\@namedef{res@ataulo-120-3.7}{-4.52}
\@namedef{res@ataulo-120-30}{-2.73}
\@namedef{res@ataulo-72-0.3}{-10.86}
\@namedef{res@ataulo-72-1}{-8.09}
\@namedef{res@ataulo-72-10}{-4.72}
\@namedef{res@ataulo-72-20}{-4.03}
\@namedef{res@ataulo-72-3}{-6.25}
\@namedef{res@ataulo-72-30}{-3.67}
\@namedef{res@ataulo-72-9.5}{-4.78}
\@namedef{res@ataulo-84-0.3}{-9.85}
\@namedef{res@ataulo-84-1}{-7.31}
\@namedef{res@ataulo-84-10}{-4.31}
\@namedef{res@ataulo-84-3}{-5.66}
\@namedef{res@ataulo-84-30}{-3.38}
\@namedef{res@ataulo-84-9.2}{-4.39}
\@namedef{res@cardI-ahi-84-10}{4.19}
\@namedef{res@cardI-ahi-84-30}{3.24}
\@namedef{res@cardI-alo-84-10}{-4.22}
\@namedef{res@cardI-alo-84-30}{-3.31}
\@namedef{res@cardI-d-84-10}{2.35}
\@namedef{res@cardI-d-84-30}{1.83}
\@namedef{res@cardI-diss-eps-maxdev}{1}
\@namedef{res@cardI-gain-84-10}{2.8}
\@namedef{res@cardI-gain-84-30}{2.5}
\@namedef{res@cardI-gain-max}{4.0}
\@namedef{res@cardI-gain-min}{2.8}
\@namedef{res@cardI-reco-1p}{94.0}
\@namedef{res@cardI-reco-3p}{74.9}
\@namedef{res@cardI-reco-eff}{78.6}
\@namedef{res@cardI-sr-84}{40.8}
\@namedef{res@cardI-sr-rel-max}{15}
\@namedef{res@cardI-sr-rel-min}{14}
\@namedef{res@cardII-d-84-10}{2.42}
\@namedef{res@cardII-d-84-30}{1.88}
\@namedef{res@cardII-reco-1p}{89.2}
\@namedef{res@cardII-reco-3p}{64.2}
\@namedef{res@cardII-reco-eff}{73.4}
\@namedef{res@cardII-sr-84}{35.4}
\@namedef{res@chan-clean-dev}{6}
\@namedef{res@chan-def-max}{3.4}
\@namedef{res@chan-def-min}{1.6}
\@namedef{res@chan-maxdev}{$-$24}
\@namedef{res@chan-maxdev-E}{120}
\@namedef{res@chan-maxdev-ch}{$\tau^-\to3\pi\nu$, $\tau^+\to\pi\pi^0\pi^0\bar\nu$}
\@namedef{res@chan-maxdev-frac}{2.6}
\@namedef{res@chan-typdev}{4}
\@namedef{res@clip1-factor-max}{4.0}
\@namedef{res@clip1-factor-min}{3.3}
\@namedef{res@clip1-gain}{8}
\@namedef{res@clip1-worsen-max}{304}
\@namedef{res@clip1-worsen-min}{227}
\@namedef{res@clip2-factor-max}{2.5}
\@namedef{res@clip2-factor-min}{2.0}
\@namedef{res@clip2-gain}{8}
\@namedef{res@clip2-worsen-max}{149}
\@namedef{res@clip2-worsen-min}{101}
\@namedef{res@clip3-factor-max}{2.0}
\@namedef{res@clip3-factor-min}{1.6}
\@namedef{res@clip3-gain}{7}
\@namedef{res@clip3-worsen-max}{102}
\@namedef{res@clip3-worsen-min}{61}
\@namedef{res@clip5-factor-max}{1.4}
\@namedef{res@clip5-factor-min}{1.2}
\@namedef{res@clip5-gain}{13}
\@namedef{res@clip5-worsen-max}{42}
\@namedef{res@clip5-worsen-min}{22}
\@namedef{res@clip8-factor-max}{1.2}
\@namedef{res@clip8-factor-min}{1.1}
\@namedef{res@clip8-gain}{18}
\@namedef{res@clip8-worsen-max}{17}
\@namedef{res@clip8-worsen-min}{7}
\@namedef{res@cms-a-ratio-10yr}{8}
\@namedef{res@cms-a-ratio-84-30}{9}
\@namedef{res@cms-d-ratio-10yr}{13}
\@namedef{res@cms-d-ratio-84-30}{15}
\@namedef{res@diss-gain-max}{13}
\@namedef{res@diss-gain-min}{9}
\@namedef{res@dissB-loss-max}{50}
\@namedef{res@dissB-loss-min}{44}
\@namedef{res@dtau-102-0.3}{5.21}
\@namedef{res@dtau-102-1}{3.88}
\@namedef{res@dtau-102-10}{2.20}
\@namedef{res@dtau-102-3}{2.96}
\@namedef{res@dtau-102-30}{1.69}
\@namedef{res@dtau-102-9.2}{2.25}
\@namedef{res@dtau-120-0.3}{4.76}
\@namedef{res@dtau-120-1}{3.50}
\@namedef{res@dtau-120-10}{1.96}
\@namedef{res@dtau-120-3}{2.65}
\@namedef{res@dtau-120-3.7}{2.51}
\@namedef{res@dtau-120-30}{1.49}
\@namedef{res@dtau-72-0.3}{6.03}
\@namedef{res@dtau-72-1}{4.50}
\@namedef{res@dtau-72-10}{2.63}
\@namedef{res@dtau-72-20}{2.24}
\@namedef{res@dtau-72-3}{3.48}
\@namedef{res@dtau-72-30}{2.04}
\@namedef{res@dtau-72-9.5}{2.66}
\@namedef{res@dtau-84-0.3}{5.59}
\@namedef{res@dtau-84-1}{4.17}
\@namedef{res@dtau-84-10}{2.42}
\@namedef{res@dtau-84-3}{3.21}
\@namedef{res@dtau-84-30}{1.88}
\@namedef{res@dtau-84-9.2}{2.47}
\@namedef{res@dtauB-102-0.3}{8.34}
\@namedef{res@dtauB-102-1}{6.25}
\@namedef{res@dtauB-102-10}{3.65}
\@namedef{res@dtauB-102-3}{4.83}
\@namedef{res@dtauB-102-30}{2.84}
\@namedef{res@dtauB-102-9.2}{3.73}
\@namedef{res@dtauB-120-0.3}{7.63}
\@namedef{res@dtauB-120-1}{5.66}
\@namedef{res@dtauB-120-10}{3.26}
\@namedef{res@dtauB-120-3}{4.34}
\@namedef{res@dtauB-120-3.7}{4.13}
\@namedef{res@dtauB-120-30}{2.52}
\@namedef{res@dtauB-72-0.3}{9.66}
\@namedef{res@dtauB-72-1}{7.27}
\@namedef{res@dtauB-72-10}{4.36}
\@namedef{res@dtauB-72-20}{3.76}
\@namedef{res@dtauB-72-3}{5.68}
\@namedef{res@dtauB-72-30}{3.44}
\@namedef{res@dtauB-72-9.5}{4.41}
\@namedef{res@dtauB-84-0.3}{8.97}
\@namedef{res@dtauB-84-1}{6.73}
\@namedef{res@dtauB-84-10}{4.01}
\@namedef{res@dtauB-84-3}{5.24}
\@namedef{res@dtauB-84-30}{3.17}
\@namedef{res@dtauB-84-9.2}{4.09}
\@namedef{res@dtauEL-102-0.3}{6.29}
\@namedef{res@dtauEL-102-1}{4.51}
\@namedef{res@dtauEL-102-10}{2.48}
\@namedef{res@dtauEL-102-3}{3.38}
\@namedef{res@dtauEL-102-30}{1.89}
\@namedef{res@dtauEL-102-9.2}{2.53}
\@namedef{res@dtauEL-120-0.3}{5.86}
\@namedef{res@dtauEL-120-1}{4.18}
\@namedef{res@dtauEL-120-10}{2.26}
\@namedef{res@dtauEL-120-3}{3.10}
\@namedef{res@dtauEL-120-3.7}{2.93}
\@namedef{res@dtauEL-120-30}{1.71}
\@namedef{res@dtauEL-72-0.3}{7.25}
\@namedef{res@dtauEL-72-1}{5.22}
\@namedef{res@dtauEL-72-10}{2.90}
\@namedef{res@dtauEL-72-20}{2.45}
\@namedef{res@dtauEL-72-3}{3.92}
\@namedef{res@dtauEL-72-30}{2.23}
\@namedef{res@dtauEL-72-9.5}{2.94}
\@namedef{res@dtauEL-84-0.3}{6.75}
\@namedef{res@dtauEL-84-1}{4.84}
\@namedef{res@dtauEL-84-10}{2.68}
\@namedef{res@dtauEL-84-3}{3.62}
\@namedef{res@dtauEL-84-30}{2.06}
\@namedef{res@dtauEL-84-9.2}{2.73}
\@namedef{res@dtauK-102-0.3}{6.27}
\@namedef{res@dtauK-102-1}{4.49}
\@namedef{res@dtauK-102-10}{2.47}
\@namedef{res@dtauK-102-3}{3.36}
\@namedef{res@dtauK-102-30}{1.89}
\@namedef{res@dtauK-102-9.2}{2.52}
\@namedef{res@dtauK-120-0.3}{5.86}
\@namedef{res@dtauK-120-1}{4.18}
\@namedef{res@dtauK-120-10}{2.26}
\@namedef{res@dtauK-120-3}{3.10}
\@namedef{res@dtauK-120-3.7}{2.93}
\@namedef{res@dtauK-120-30}{1.72}
\@namedef{res@dtauK-72-0.3}{7.20}
\@namedef{res@dtauK-72-1}{5.17}
\@namedef{res@dtauK-72-10}{2.87}
\@namedef{res@dtauK-72-20}{2.42}
\@namedef{res@dtauK-72-3}{3.88}
\@namedef{res@dtauK-72-30}{2.20}
\@namedef{res@dtauK-72-9.5}{2.90}
\@namedef{res@dtauK-84-0.3}{6.72}
\@namedef{res@dtauK-84-1}{4.81}
\@namedef{res@dtauK-84-10}{2.65}
\@namedef{res@dtauK-84-3}{3.60}
\@namedef{res@dtauK-84-30}{2.04}
\@namedef{res@dtauK-84-9.2}{2.71}
\@namedef{res@dtauS50-102-0.3}{5.67}
\@namedef{res@dtauS50-102-1}{4.21}
\@namedef{res@dtauS50-102-10}{2.31}
\@namedef{res@dtauS50-102-3}{3.17}
\@namedef{res@dtauS50-102-30}{1.74}
\@namedef{res@dtauS50-102-9.2}{2.36}
\@namedef{res@dtauS50-120-0.3}{5.17}
\@namedef{res@dtauS50-120-1}{3.77}
\@namedef{res@dtauS50-120-10}{2.04}
\@namedef{res@dtauS50-120-3}{2.80}
\@namedef{res@dtauS50-120-3.7}{2.65}
\@namedef{res@dtauS50-120-30}{1.54}
\@namedef{res@dtauS50-72-0.3}{6.51}
\@namedef{res@dtauS50-72-1}{4.93}
\@namedef{res@dtauS50-72-10}{2.80}
\@namedef{res@dtauS50-72-20}{2.36}
\@namedef{res@dtauS50-72-3}{3.78}
\@namedef{res@dtauS50-72-30}{2.14}
\@namedef{res@dtauS50-72-9.5}{2.84}
\@namedef{res@dtauS50-84-0.3}{6.04}
\@namedef{res@dtauS50-84-1}{4.53}
\@namedef{res@dtauS50-84-10}{2.56}
\@namedef{res@dtauS50-84-3}{3.45}
\@namedef{res@dtauS50-84-30}{1.96}
\@namedef{res@dtauS50-84-9.2}{2.61}
\@namedef{res@dtauclip1-102}{7.91}
\@namedef{res@dtauclip1-120}{7.91}
\@namedef{res@dtauclip1-72}{8.60}
\@namedef{res@dtauclip1-84}{8.09}
\@namedef{res@dtauclip2-102}{5.17}
\@namedef{res@dtauclip2-120}{4.88}
\@namedef{res@dtauclip2-72}{5.28}
\@namedef{res@dtauclip2-84}{5.16}
\@namedef{res@dtauclip3-102}{4.10}
\@namedef{res@dtauclip3-120}{3.95}
\@namedef{res@dtauclip3-72}{4.25}
\@namedef{res@dtauclip3-84}{4.01}
\@namedef{res@dtauclip5-102}{2.97}
\@namedef{res@dtauclip5-120}{2.78}
\@namedef{res@dtauclip5-72}{3.21}
\@namedef{res@dtauclip5-84}{2.99}
\@namedef{res@dtauclip8-102}{2.49}
\@namedef{res@dtauclip8-120}{2.29}
\@namedef{res@dtauclip8-72}{2.80}
\@namedef{res@dtauclip8-84}{2.62}
\@namedef{res@eps-excl-dy}{\num{2.15e-05}}
\@namedef{res@epsratio-dd-high}{0.34}
\@namedef{res@epsratio-dd-low}{0.27}
\@namedef{res@epsratio-sd-high}{0.60}
\@namedef{res@epsratio-sd-low}{0.41}
\@namedef{res@gain-1}{22}
\@namedef{res@gain-10}{26}
\@namedef{res@gain-30}{27}
\@namedef{res@gain-step-max}{11}
\@namedef{res@gain-step-min}{8}
\@namedef{res@hd-fsd}{0.8}
\@namedef{res@hd-n30}{\num{1.4e+03}}
\@namedef{res@hd-n30-err}{\num{1e+03}}
\@namedef{res@hd-nacc}{3\,447}
\@namedef{res@hd-nch}{21}
\@namedef{res@hd-p0}{\num{4e-04}}
\@namedef{res@hd-rel-low}{1.3}
\@namedef{res@kappa-a-84-10}{4.3}
\@namedef{res@kappa-t-84-10}{4.4}
\@namedef{res@lscale-max}{0.26}
\@namedef{res@lscale-min}{0.23}
\@namedef{res@lumi-equiv}{3.5}
\@namedef{res@mw-3p-high}{45}
\@namedef{res@mw-3p-high-nmw}{80}
\@namedef{res@mw-3p-low}{73}
\@namedef{res@mw-eff}{74}
\@namedef{res@mw-eff-nmw}{81}
\@namedef{res@mw-lim-gain}{6}
\@namedef{res@mw-lim-gain-hi}{7}
\@namedef{res@mw-sr}{35.8}
\@namedef{res@mw-sr-gain}{28}
\@namedef{res@mw-sr-nmw}{45.8}
\@namedef{res@pu-lim-w02}{23}
\@namedef{res@pu-mu-84}{590}
\@namedef{res@pu-n-84}{8.3}
\@namedef{res@pu-p0-84}{\num{3e-04}}
\@namedef{res@pu-p0-84-w02}{44}
\@namedef{res@pu-sl}{57}
\@namedef{res@pu-w50-84}{168}
\@namedef{res@pu-w50-f12hl}{35}
\@namedef{res@pu-w50-f20}{789}
\@namedef{res@reco-eff}{73.4}
\@namedef{res@reco-fake-d}{282\,133}
\@namedef{res@reco-fake-n}{10}
\@namedef{res@reco-mode}{82.3}
\@namedef{res@reco-prong}{99.2}
\@namedef{res@rv-1p-none}{9}
\@namedef{res@rv-1p-ok}{89}
\@namedef{res@rv-3p-as1p}{1.6}
\@namedef{res@rv-3p-none}{34}
\@namedef{res@rv-3p-ok}{64}
\@namedef{res@rv-eff-high}{75}
\@namedef{res@rv-eff-low}{73}
\@namedef{res@rv-pi0-as1p}{19}
\@namedef{res@rv-pi0-core}{69}
\@namedef{res@rv-pi0-none}{30}
\@namedef{res@rv-pi0-ok}{51}
\@namedef{res@rv-res-1p}{0.9}
\@namedef{res@rv-res-3p}{0.6}
\@namedef{res@rv-res-pi0}{2.2}
\@namedef{res@s0-again-84-30}{6}
\@namedef{res@s0-ahi-84-30}{3.18}
\@namedef{res@s0-alo-84-30}{-3.15}
\@namedef{res@s0-d-84-30}{1.77}
\@namedef{res@s0-dgain-84-30}{6}
\@namedef{res@s2-ap-max}{0.87}
\@namedef{res@s2-ap-min}{0.85}
\@namedef{res@s2-sm-max}{0.96}
\@namedef{res@s2-sm-min}{0.93}
\@namedef{res@sc-mg-max}{1.056}
\@namedef{res@sc-mg-min}{1.034}
\@namedef{res@sm-lowmass-frac}{80}
\@namedef{res@sr-eff-84}{35.4}
\@namedef{res@ten-a-best}{4.1}
\@namedef{res@ten-a-worst}{4.9}
\@namedef{res@ten-d-best}{2.24}
\@namedef{res@ten-d-worst}{2.66}
\@namedef{res@xs-base-84}{89.1}
\@namedef{res@xs-dy-84}{147}
\@namedef{res@xs-fitdev}{0.03}
\@namedef{res@xs-npts}{27}
\@namedef{res@xs-r-a5}{0.3}
\@namedef{res@xs-r-d5}{0.1}
\@namedef{res@xs-ww-84}{1.75}
\@namedef{res@y-bkg-150}{1\,031}
\@namedef{res@y-bkg-1tev}{8.5}
\@namedef{res@y-bkg-rel-el}{2.5}
\@namedef{res@y-bkg-rel-tot}{0.9}
\@namedef{res@y-diss-ratio}{1.9}
\@namedef{res@y-npa-1tev}{122}
\@namedef{res@y-npa-3tev}{10}
\@namedef{res@y-npa-rel-150}{1.2}
\@namedef{res@y-npa-rel-1tev}{29}
\@namedef{res@y-npa-rel-3tev}{2.3}
\@namedef{res@y-npd-rel-3tev}{2.2}
\@namedef{res@y-sm-below150}{70}
\@namedef{res@y-smdiss-150}{78\,092}
\@namedef{res@y-smel-150}{41\,062}
\@namedef{res@y-smtot-150}{119\,154}
\@namedef{res@y-smtot-1tev}{427}
\@namedef{res@y-smtot-3tev}{4.6}
\@namedef{res@yield-dy-84-30}{80}
\@namedef{res@yield-sm-84-30}{136\,165}
\@namedef{res@yield-ww-84-30}{951}
\makeatother
\newcommand{\res}[1]{\ifcsname res@#1\endcsname\csname res@#1\endcsname\else{\color{red}??#1??}\fi}

